Language-guided Robust Navigation for Mobile Robots in Dynamically-changing Environments

In this paper, we develop an embodied AI system for human-in-the-loop navigation with a wheeled mobile robot. We propose a direct yet effective method of monitoring the robot's current plan to detect changes in the environment that impact the intended trajectory of the robot significantly and then query a human for feedback. We also develop a means to parse human feedback expressed in natural language into local navigation waypoints and integrate it into a global planning system, by leveraging a map of semantic features and an aligned obstacle map. Extensive testing in simulation and physical hardware experiments with a resource-constrained wheeled robot tasked to navigate in a real-world environment validate the efficacy and robustness of our method. This work can support applications like precision agriculture and construction, where persistent monitoring of the environment provides a human with information about the environment state.

==> figures/factory_map.tex <==
\begin{figure*}[!t]
    \centering
    \subfloat[Gazebo Environment]{
        \reflectbox{
                \frame{\includegraphics[angle=180,width=0.4\linewidth]{images/maps/factory_gazebo.png}}
        }
    }%
    \subfloat[RGB Map]{
        \reflectbox{
            \includegraphics[angle=90,width=0.4\linewidth]{images/maps/factory_rgb.png}
        }
    }%
    \caption{A comparison between top down view of the factory environment rendered in Gazebo and the corresponding RGB map created during our map construction process. Note that while the major features agree, there are still noisy edges caused by sensor noise which was not present in previous simulations.}%
\label{fig:factory_map}
\end{figure*}

==> figures/graph_construction.tex <==
\begin{figure}[!t]
\vspace{6pt}
\centering
\includegraphics[trim={0cm, 1.25cm, 0cm, 1.25cm},clip,width=\columnwidth]{images/Graph Construction.pdf}
\vspace{-18pt}
\caption{Here we show, an example graph construction for \textit{Waypoint Selection Module}, with edge weights omitted for clarity. Note that nodes are connected with an edge if the waypoints belong to sequential descriptions. After construction, we find the shortest path to each waypoint corresponding to the final description and pick the route to the closest waypoints as our modified trajectory, shown in green.}
\label{fig:graph_construction}
\end{figure}

==> figures/physcial_system_traj.tex <==
\begin{figure*}
    \centering
    \subfloat[Route 1]{
        \frame{\includegraphics[trim=120 50 110 60, clip, width=0.3\textwidth]{images/physical/system_tests_r0.png}}
    }%
    \subfloat[Route 2]{
        \frame{\includegraphics[trim=120 50 110 60, clip, width=0.3\textwidth]{images/physical/system_tests_r1.png}}
    }%
    \subfloat[Route 3]{
        \frame{\includegraphics[trim=120 50 110 60, clip, width=0.3\textwidth]{images/physical/system_tests_r2.png}}
    }%
    \caption{Visualized results of our real-world experiments, with each trial drawn in blue and the ground truth trajectory drawn in green. We note that route 2 has a higher mean than the other routes since it consistently picks a final waypoint far from the ground truth endpoint.}%
    \label{fig:physical_system_traj}
\end{figure*}

==> figures/physical_map.tex <==
\begin{figure}[!t]
    \centering
    \reflectbox{\includegraphics[angle=90,width=0.8\columnwidth]{images/maps/wch_floor1_rgb.png}}
    \caption{RGB visualization of the map we collected in our real-world experiments. The ground plane is not mapped , due to differences in the physical RGBD camera vs the simulated camera. Since this is collected in the real-world we have no ground truth rendering to compare to.}
    \label{fig:physical_map}
\end{figure}

==> figures/simulated_lang_traj.tex <==
\begin{figure*}[!t]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \subfloat[Small House]{
        \subfloat[Route 1]{
            \frame{\includegraphics[trim=115 100 102 90, clip, width=0.3\textwidth]{images/simulation/small_house_lang_nav_r0.png}}
        }%
        \subfloat[Route 2]{
            \frame{\includegraphics[trim=115 100 102 90, clip, width=0.3\textwidth]{images/simulation/small_house_lang_nav_r1.png}}
        }%
        \subfloat[Route 3]{
            \frame{\includegraphics[trim=115 100 102 90, clip, width=0.3\textwidth]{images/simulation/small_house_lang_nav_r2.png}}
        }%
    }
    \vspace{-9pt}
    \subfloat[Factory]{
        \subfloat[Route 1]{
            \frame{\includegraphics[trim=120 110 110 110, clip, width=0.3\textwidth]{images/simulation/factory_lang_nav_r0.png}}
        }%
        \subfloat[Route 2]{
            \frame{\includegraphics[trim=120 110 110 110, clip, width=0.3\textwidth]{images/simulation/factory_lang_nav_r1.png}}
        }%
        \subfloat[Route 3]{
            \frame{\includegraphics[trim=120 110 110 110, clip, width=0.3\textwidth]{images/simulation/factory_lang_nav_r2.png}}
        }%
    }
    \caption{Visualized results of our language navigation ablation study, with each trajectory of our method drawn in blue and the ground truth drawn in green. Note that the cases with the routes with high RMSE include erroneous waypoints, which bring part of the trajectory away from the ground truth.}%
\label{fig:simulated_lang_traj}
\end{figure*}

==> figures/simulated_system_traj.tex <==
\begin{figure*}[!t]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \subfloat[Small House]{
        \subfloat[Route 1]{
            \frame{\includegraphics[trim=115 100 102 90, clip, width=0.3\textwidth]{images/simulation/small_house_system_test_r0.png}}
        }%
        \subfloat[Route 2]{
            \frame{\includegraphics[trim=115 100 102 90, clip, width=0.3\textwidth]{images/simulation/small_house_system_test_r1.png}}
        }%
        \subfloat[Route 3]{
            \frame{\includegraphics[trim=115 100 102 90, clip, width=0.3\textwidth]{images/simulation/small_house_system_test_r2.png}}
        }%
    }
    \vspace{-9pt}
    \subfloat[Factory]{
        \subfloat[Route 1]{
            \frame{\includegraphics[trim=120 110 110 110, clip, width=0.3\textwidth]{images/simulation/factory_system_test_r0.png}}
        }%
        \subfloat[Route 2]{
            \frame{\includegraphics[trim=120 110 110 110, clip, width=0.3\textwidth]{images/simulation/factory_system_test_r1.png}}
        }%
        \subfloat[Route 3]{
            \frame{\includegraphics[trim=120 110 110 110, clip, width=0.3\textwidth]{images/simulation/factory_system_test_r2.png}}
        }%
    }\\
    \caption{Visualized results of our simulation experiments. Each trajectory of our method is drawn in blue and the ground truth trajectory is drawn in green. Note that the cases with the routes with high RMSE include erroneous waypoints, which bring part of the trajectory away from the ground truth.}%
\label{fig:simulated_system_traj}
\end{figure*}

==> figures/small_house_map.tex <==
\begin{figure}[!t]
\vspace{6pt}
    \centering
    \subfloat[]{%[Gazebo Environment]{
        \reflectbox{
                \frame{\includegraphics[angle=180,width=0.65\linewidth]{images/maps/small_house_gazebo.png}}
        }
    }%
    \\
    \subfloat[]{%[RGB Map]{
        \reflectbox{
            \includegraphics[angle=90,width=0.65\linewidth]{images/maps/small_house_rgb.png}
        }
    }%
    \caption{(a) Top-down view of the small house environment rendered in Gazebo and (b) the corresponding RGB map created during our map construction process. Note that while the major features agree, there can still be inexact edges caused by sensor noise.}% which was not present in previous simulations.}%
\label{fig:small_house_map}
\end{figure}

==> sections/3_problem.tex <==
\section{Problem Statement}\label{problem}
Given a sequence of $(x, y, \theta)$ navigation waypoints, defined by a human operator, the robot must plan a route based on a priori knowledge of the environment in the form of an occupancy map. During execution, the robot must continuously monitor the environment for changes that may render the initial trajectory invalid. Upon detecting such changes, the robot queries the human operator for feedback to adapt its trajectory. The feedback is provided in natural language, consisting of a sequence of descriptive phrases corresponding to specific locations within the environment. The robot must then process and integrate this feedback to modify its trajectory to account for environmental changes.



%Since the environment is assumed to be known, an obstacle map and a semantic features map have been constructed. Obstacle map can be constructed using widely available mapping tools\cite{grisetti2007gmapping} tools with a 2D lidar. To construct a semantic feature map, we assume the robot is equipped with an RGBD camera, which can collect data while the obstacle map is being created. These can be localized relative to the obstacle map, by matching each RGBD image to the most recent lidar scan and aligning the scan with the obstacle map. Following the method proposed in \cite{huang2023vlmaps} we extract dense semantic feature vectors from the RGB channels and use the depth information to perform 3D reconstruction, associating each 3D point with a $d$ dimensional feature vector. The points are then projected the ground plane to create a 2D map of semantic features $f\in\mathbb{R}^{H\times W\times d}$, where $H$ and $W$ are the height and width of the feature map.

%Throughout the rest of this work, we will assume that there exists some nominal trajectory, defined by a series of navigation waypoints manually entered by a person. This trajectory will be created with the knowledge of the pre-existing map, however there will be some changes to the environment which effect the robots trajectory. The robot needs to decide when these changes are significant enough to require human feedback. When human feedback is given it will come in the form of natural language, which for this work we further limit to be descriptions of the visual appearance of different locations on the map. From this feedback a new set of waypoints needs to be generated to guide the

==> tables/initial_results.tex <==
\begin{table}[]
    \centering
    \caption{}
    \begin{tabular}{c|c}
         RMSE &  $4.041\pm0.001$\\
         SR & $0.66$
    \end{tabular}
    \label{tab:my_label}
\end{table}

%Trial 1,  4.074846, Success
%Trial 2, 16.890213, Failure
%Trial 3,  4.007151, Success

==> tables/physical_system_test.tex <==
\begin{table}[!t]
    \vspace{-6pt}
    \centering
    \caption{Physical experiment system test results}
    \begin{tabular}{ccccc}
        \toprule
        & RMSE & SR\\
        \midrule
        Route 1 & $0.375\pm0.151$ & $0.63$\\
        Route 2 & $1.850\pm2.425$ & $0.83$\\
        Route 3 & $0.668\pm0.064$ & $1.00$\\
        Average & $0.964\pm1.541$ & $0.79$\\
        \bottomrule
    \end{tabular}
    \vspace{0.2em}
    \label{tab:physical_system_test}
\end{table}

==> tables/simulation_lang_nav.tex <==
\begin{table}[h]
    \centering
    \caption{Ablation Study Results.}
    \begin{tabular}{ccc}
        \toprule
        & \multicolumn{1}{c}{Small House} & \multicolumn{1}{c}{Factory}\\
        \cmidrule(lr){1-2}\cmidrule(lr){2-3} 
        & RMSE & RMSE\\
        \midrule
        Route 1 & $0.905\pm0.622$ & $0.332\pm0.005$\\
        Route 2 & $1.298\pm1.239$ & $4.110\pm2.685$\\
        Route 3 & $1.443\pm0.570$ & $2.299\pm0.016$\\
        Average & $1.215\pm0.895$ & $2.247\pm2.187$\\
        \bottomrule
    \end{tabular}
    \vspace{0.2em}
    \label{tab:simulation_lang_nav}
\end{table}

==> tables/simulation_system_test.tex <==
\begin{table}[ht]
    \centering
    \caption{Simulation experiments system test results}
    \begin{tabular}{ccccc}
        \toprule
        & \multicolumn{2}{c}{Small House} & \multicolumn{2}{c}{Factory}\\
        \cmidrule(lr){2-3}\cmidrule(lr){4-5} 
        & RMSE & SR & RMSE & SR\\
        \midrule
        Route 1 & $0.507\pm0.100$ & $1.00$ & $0.324\pm0.046$ & $1.00$\\
        Route 2 & $0.442\pm0.061$ & $1.00$ & $3.056\pm1.881$ & $1.00$\\
        Route 3 & $0.460\pm0.091$ & $1.00$ & $0.989\pm1.215$ & $0.80$\\
        Average & $0.470\pm0.090$ & $1.00$ & $1.456\pm1.739$ & $0.93$\\
        \bottomrule
    \end{tabular}
    \vspace{0.2em}
    \label{tab:simulation_system_test}
\end{table}
